Read it Twice: Towards Faithfully Interpretable Fact Verification by Revisiting Evidence

Real-world fact verification task aims to verify the factuality of a claim by retrieving evidence from the source document. The quality of the retrieved evidence plays an important role in claim verification. Ideally, the retrieved evidence should be faithful (reflecting the model's decision-making process in claim verification) and plausible (convincing to humans), and can improve the accuracy of verification task. Although existing approaches leverage the similarity measure of semantic or surface form between claims and documents to retrieve evidence, they all rely on certain heuristics that prevent them from satisfying all three requirements. In light of this, we propose a fact verification model named ReRead to retrieve evidence and verify claim that: (1) Train the evidence retriever to obtain interpretable evidence (i.e., faithfulness and plausibility criteria); (2) Train the claim verifier to revisit the evidence retrieved by the optimized evidence retriever to improve the accuracy. The proposed system is able to achieve significant improvements upon best-reported models under different settings.

==> subfiles/2_related.tex <==
% % \input{tables/dataset}

% \section{Related Work}
% \label{related}

% \subsection{Fact-Checking Datasets} 
% % 
% Table~\ref{tab:dataset} summarized fact-checking dataset by grouping them into two types: real-world and synthetic \cite{guo2021}. 
% % Existing datasets can be grouped into two types: real-world and synthetic ~\citep{guo2021}. 
% Real-world dataset consists of claims that originates from the media ecosystem and are fact-checked by dedicated agencies (e.g. PolitiFact). Synthetic datasets contain claims created artificially by mutating sentences from Wiki articles. Early efforts predicted the veracity solely based on the claims or with metadata \cite{Rashkin2017TruthOV, Wang2017LiarLP}, but studies show that predictions that do not consider evidence fails to identify misinformation \cite{Schuster2020TheLO}. Therefore, synthetic datasets \cite{Thorne18Fact,jiang2020hover,vitaminc2021} considered Wikipedia as the source of evidence and annotated the sentences from articles as evidence.  
% % Although these datasets incorporated evidence, they restricted world knowledge to a single source (i.e. Wikipedia), ignoring the challenge of collecting evidence from heterogeneous sources. 
% However, these efforts restricted world knowledge to a single source (i.e. Wikipedia), which is not ideal to develop systems that collect evidence from heterogeneous sources. On the other hand, real-world efforts~\cite{Hanselowski2019ARA, kotonya2020health} extracted summaries accompanying fact-checking articles about the claims as evidence. Nonetheless, using fact-checking articles is not realistic, as they are not available during inference. To address this issue, other datasets~\cite{Augenstein2019MultiFCAR, gupta-srikumar-2021-x} included search snippets generated by Google as evidence. Unlike prior real-world efforts, we propose to directly incorporate retrieved documents to provide more information for better verification.


% \subsection{Fact-Checking Systems} 
% When verifying synthetic claims, systems often operate as a pipeline consisting of an evidence extraction module and a verification module. Relevant articles are first retrieved from the Wikipedia dump by using entity linking, or TF-IDF~\citep{hanselowski-etal-2018-ukp,Thorne18Fact}.  After obtaining the evidence sentences, a textual entailment model is applied for the claim verification~\citep{luken-etal-2018-qed, Nie2019CombiningFE}. Recent systems employ graph-based models to aggregate evidence. This allows the verification of more complex claims where several pieces of information can be combined~\citep{Zhou2019GEARGE, Liu2020KernelGA, Zhong2020ReasoningOS, schlichtkrull2020}. Due to the difficulty of annotating evidence under real-world scenarios, most systems assume the evidence sentences are given, ignoring the challenge of evidence extraction~\citep{Hanselowski2019ARA,Augenstein2019MultiFCAR,kotonya2020health,gupta-srikumar-2021-x}. Different from these methods, we propose to model the evidence extraction as a latent variable. Such a design enables our system to extract evidence from web sources and validate real-world claims based on evidence found on the Internet. 


% % When verifying synthetic claims, systems often operate as a pipeline consisting of an evidence extraction module and a verification module~\citep{guo2021}, as the annotation of evidence sentences are provided. Relevant articles are first retrieved from the Wikipedia dump by using entity linking, or TF-IDF~\citep{hanselowski-etal-2018-ukp,Thorne18Fact}. Then a fine-grained module can be trained to extract related sentences from retrieved articles~\citep{nie-etal-2019-revealing, Nie2019CombiningFE,Liu2020KernelGA}. After obtaining the evidence sentences, a textual entailment model is applied for the claim verification~\citep{luken-etal-2018-qed, Nie2019CombiningFE}. Recent systems employ graph-based models to aggregate evidence. This allows the verification of more complex claims where several pieces of information can be combined~\citep{Zhou2019GEARGE, Liu2020KernelGA, Zhong2020ReasoningOS, schlichtkrull2020}. Due to the difficulty of annotating evidence under real-world scenarios, most systems assume the evidence sentences are given, ignoring the challenge of evidence extraction~\citep{Hanselowski2019ARA,Augenstein2019MultiFCAR,kotonya2020health,gupta-srikumar-2021-x}. Different from these methods, we propose to model the evidence extraction as a latent variable. Such a design enables our system to extract evidence from web-sources and validate real-world claims based on evidence found on the Internet. 

% % Some early work does not include evidence retrieval at all, performing verification purely on the basis of surface forms and metadata~\citep{Wang2017LiarLP,Rashkin2017TruthOV,Dungs2018CanRS}. Recently \citet{lee-etal-2020-language} 
% % considered using the information stored in the weights of a large pretrained language model -- BERT~\citep{Devlin2019BERTPO} -- as the only source of evidence, as it has been shown competitive in knowledge base completion \citep{petroni-etal-2019-language}.
% % Without explicitly considering evidence such approaches are likely to propagate biases learned during training, and render justification production impossible~\citep{lee-etal-2021-towards,PanCXKW20}.


% % Similarly, evidence can be re-ranked implicitly during verification in late-fusion systems
% % %late-fusion strategies where evidence is re-ranked implicitly as part of the verification system have also been proposed
% % ~\citep{ma-etal-2019-sentence, schlichtkrull2020}.


% %The primary challenge for retrieval systems is scale -- the number of articles in potential information sources such as Wikipedia, LexisNexis, or Google News is massive. Retrieval modules are therefore very limited in how much processing can be spent on each potential piece of evidence. This challenge has been addressed through  various
% % Recently, dense retrievers employing learned representations and fast dot-product indexing~\citep{johnson2017faiss} have shown strong performance~\citep{lewis2020retrieval, maillard-etal-2021-multi}. %Efficient retrieval often comes as the expense of precision. To alleviate this,

% % An alternative approach was proposed by \citet{Fan2020GeneratingFC}, who retrieved evidence using question generation and question answering via search engine results. 
% % Some work avoids retrieval by making a \textit{closed-domain assumption} and %, i.e.\ assuming access to an oracle retriever, and 
% % evaluating in a setting where appropriate evidence has already been found~\citep{Ferreira2016EmergentAN,Chen2020TabFactAL, zhong-etal-2020-logicalfactchecker, yang-etal-2020-program, eisenschlos-etal-2020-understanding}; this, however, is unrealistic. Finally, \citet{allein2021time} took into account the timestamp of the evidence in order to improve veracity prediction accuracy.

% % What to do with evidence


==> tables/classes.tex <==
\begin{table}[t]
\centering
\caption{F1 Performance against Veracity Classes.}
\vspace{-4mm}
\scalebox{0.8}{
\begin{tabular}{l|cccc|c}
\thickhline
\multicolumn{1}{l|}{\multirow{1}{*}{Classes}} & \multicolumn{1}{c}{No Evidence} & \multicolumn{1}{c}{Hybrid Ranker}& \multicolumn{1}{c}{Latent}& \multicolumn{1}{c|}{{\modelname}}& \multicolumn{1}{c}{Gold Evidence}
\\ 
\midrule 
\multicolumn{1}{l|}{Sup} & 48.42 & 60.55  & 63.34 & \textbf{69.54} & 82.49 \\
\multicolumn{1}{l|}{Ref} & 75.51 & 83.24 &  85.83 & \textbf{87.75} & 95.12\\
\multicolumn{1}{l|}{NEI} & 33.64 & 42.28 & 45.23 &\textbf{49.74}   &  55.22\\
\thickhline
\end{tabular}}
\label{tab:classes}
\vspace{-5mm}
\end{table}

==> tables/statics.tex <==
\begin{table}
\centering
\caption{Dataset split sizes and statistics for CHEF.}
\vspace{-4mm}
\scalebox{0.85}{
\begin{tabular}{lcccc}
\toprule
Split & SUP & REF & NEI & Total \\
\midrule
Train & 2,877 & 4,399 & 776 & 8,002 \\
Dev & 333 & 333 & 333 & 999 \\
Test & 333 & 333 & 333 & 999 \\
\midrule
\midrule
\multicolumn{4}{l}{Avg \#Words in the Claim} & 28 \\
\multicolumn{4}{l}{Avg \#Words in the Google Snippets} & 68 \\
\multicolumn{4}{l}{Avg \#Words in the Gold Evidence Sentences} & 126 \\
\multicolumn{4}{l}{Avg \#Words in the Source Documents} & 3,691 \\
\bottomrule
\end{tabular}}
\label{tab:split}
\vspace{-5mm}
\end{table}
